Eliciting Model Steering Interactions from Users via Data and Visual Design Probes

Domain experts increasingly use automated data science tools to incorporate machine learning (ML) models in their work but struggle to "debug" these models when they are incorrect. For these experts, semantic interactions can provide an accessible avenue to guide and refine ML models without having to programmatically dive into its technical details. In this research, we conduct an elicitation study using data and visual design probes to examine if and how experts with a spectrum of ML expertise use semantic interactions to update a simple classification model. We use our design probes to facilitate an interactive dialogue with 20 participants and codify their interactions as a set of target-interaction pairs. Interestingly, our findings revealed that many targets of semantic interactions do not directly map to ML model parameters, but instead aim to augment the data a model uses for training. We also identify reasons that participants would hesitate to interact with ML models, including burdens of cognitive load and concerns of injecting bias. Unexpectedly participants also saw the value of using semantic interactions to work collaboratively with members of their team. Participants with less ML expertise found this to be a useful mechanism for communicating their concerns to ML experts. This was an especially important observation, as our study also shows the different needs that correspond to diverse ML expertise. Collectively, we demonstrate that design probes are effective tools for proactively gathering the affordances that should be offered in an interactive machine learning system.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tex/abstract.tex <==
\begin{abstract}
Domain experts increasingly use automated data science tools to incorporate machine learning (ML) models in their work but struggle to ``debug'' these models when they are incorrect. For these experts, semantic interactions can provide an accessible avenue to guide and refine ML models without having to programmatically dive into its technical details.  In this research, we conduct an elicitation study using data and visual design probes to examine if and how experts with a spectrum of ML expertise use semantic interactions to update a simple classification model. We use our design probes to facilitate an interactive dialogue with 20 participants and codify their interactions as a set of target-interaction pairs. Interestingly, our findings revealed that many targets of semantic interactions do not directly map to ML model parameters, but instead aim to augment the data a model uses for training.  We also identify reasons that participants would hesitate to interact with ML models, including burdens of cognitive load and concerns of injecting bias.  Unexpectedly participants also saw the value of using semantic interactions to work collaboratively with members of their team.  Participants with less ML expertise found this to be a useful mechanism for communicating their concerns to ML experts. This was an especially important observation, as our study also shows the different needs that correspond to diverse ML expertise.  Collectively, we demonstrate that design probes are effective tools for proactively gathering the affordances that should be offered in an interactive machine learning system.
\end{abstract}

%Semantic interactions allow people to update a machine learning model by interacting more directly with the data to update the model. For people without a  background in machine learning (ML) or data science (DS), semantic interactions may offer a more accessible way to guide machine learning models without being forced to dive into the model’s technical details. However, prior research has not studied the different responses of ML and non-ML practitioners to semantic interactions. Moreover, there is also little research on the effects of different visual encodings on the affordances of semantic interactions. Here, we conduct an elicitation study with several visual design probes to explore the relationships between visual encodings, ML/DS expertise, and semantic interactions. We delineate a space of action and intervention pairs of different mark types and compare the frequency of such actions among 20 participants, half classified as ML practitioners and half not. Our study also identifies different models of collaborative updating procedures between humans and machine learning models. Finally, we show how semantic interactions can facilitate human-machine collaboration and human-human collaboration between people with different degrees of expertise in machine learning. Our approach and its findings have implications for data science technology that seeks to become more accessible to those without extensive training in machine learning. 



==> tex/pilot_study.tex <==
%\subsection{Pilot Study }
\label{sec:pilot_study}
%
%In addition to refining aspects of our design probe (i.e., spelling errors, complex flow, design inconsistencies), the pilot study also quantified the ordering effect of our visual probes. % The first was that 
%Specifically  table elicited quite strong reactions from participants, especially if it was the first visualization. We also observed that participants saw similarities between the scatter chart and the dot chart, which further influenced their responses. We decided to mitigate such a potentially strong confound in our analysis by grouping the table (T), bar chart (B), scatter chart (S), and a dot chart (D) into two sets and varying the order in which they would be presented to the participants. While there were a total of 24 possible orders, we settled on four that we felt gave good coverage of these possible combinations: [(TS)(DB)], [(TD)(BS)], [(ST)(DB)], [(DB)(ST)].  Given these presentation orders, our study would need to recruit at least eight participants (4 ML and 4 non-ML). We wanted at least each order to be viewed twice within each group, which resulted in a minimum study size of 16 participants.



%it surfaced the effects of visualization ordering on participant response. Digging into this effect helped us determine a minimal number of participants for the full study. Second, the pilot study sensitized us to the kinds of feedback participants wanted to provide (semantic interactions and UX improvements). Finally, it provided us with a preliminary nomenclature for intervention-action pairs. 

%\vspace{1mm}
%\noindent\textbf{Effects of Visualization Order.}\label{subsec:pilot_order}

%\vspace{1mm}
%\noindent\textbf{Semantic Interactions and UX Improvements.}\label{subsec:pilot_learn_ux}
%When pilot participants were engaging with the data visualizations, they commented not only on how their actions were intended to refine the model but also how it would make it easier for them to do so. From this observation, we characterized two types of findings, \textit{Semantic Actions} and \textit{UX Improvements}. In our study \textit{Semantic Actions} refine machine learning models via direct manipulation of a data encoding mark's visual channels. %They are represented in~\autoref{fig:interactive_notion} as acting on model parameters via $\erelbar{02}$. %For example, if a data visualization is using size to encode the classification probability of the model, then when a participant changes the size of the point, they are providing input to the model on how confident it should be in its prediction. When the machine learning model updates, it may also try to fit itself to predict that data point with a specific probability provided by the user.   
%The primary goal of our elicitation study was to uncover these semantic interactions for a variety of visual encodings, while \textit{UX  Improvements} are elements of the visual and interaction design of a (hypothetical) system that would help the participant review and modify machine learning model results. For example, participants wanted to sort movies by classification probability, filter on a specific subset of the movie, or even highlight changes. These interactions do not necessarily generate data usable to a machine learning model, even though they modify the visualization, so they do not fall into the narrow definition of semantic interactions we use here.  We discuss UX improvements as well, but not to the same extent as semantic interactions.

%\vspace{1mm}
%\noindent\textbf{Interventions and Actions}\label{subsec:pilot_intervene_act}
%The pilot initiated the idea of a set of intervention-action pairs. The \textit{interventions} are the attributes of the initial dataset or results of the model that a participant modifies. The \textit{actions} are the semantic interactions the participant uses to modify. For example, when a participant wishes to modify the classification probability, the point of intervention is the probability and the size channel that encodes it, whereas the action changes the size of the mark. Primed by the pilot study, we extensively elaborated upon this idea within the full study.  

%From the pilot study we established that refinement actions could be described as a set of intervention-action pairs. The \textit{interventions} are the attributes of $D$ or $R$ that a person modifies and \textit{actions} are how they do it. As an example, when a participant wishes to modify the classification probability, the point of intervention is the probability and the size channel that encodes it, whereas the action is changing the size of the mark. We derived an initial set of intervention-action pairs in the pilot and expanded on these in the full study.




==> tex/scratch.tex <==
\textbf{GPT suggestions:}

Persuasive

Semantic interactions are a way to directly manipulate data visualizations in order to update a machine learning model. They offer a more accessible way for people without a background in machine learning or data science to guide the model. However, there is limited research on whether the affordances offered by semantic interactions meet the expectations of domain experts who work with ML models. We conducted an elicitation study using visual design probes to elicit how semantic interactions refine ML models from participants. In semi-structured interviews with 20 participants, we captured and summarized semantic interactions as a set of target-action pairs. Additionally, we found that participants expected a visual analytics system to perform speculative execution in response to their semantic interaction; they wanted be able to review the effects of their interaction on the model before making any changes.


Professional

Semantic interactions are a way to directly manipulate data visualizations in order to update a machine learning model. They offer a more accessible way for people without a background in machine learning or data science to guide the model. However, there is limited research on whether the affordances offered by semantic interactions meet the expectations of domain experts who work with ML models. We conducted an elicitation study using visual design probes to elicit how semantic interactions refine ML models from participants. In semi-structured interviews with 20 participants, we captured and summarized semantic interactions as a set of target-action pairs. Additionally, we found that participants expected a visual analytics system to perform speculative execution in response to their semantic interaction; they wanted be able to review the effects of their interaction on the model before making any changes.


Blog post - professional
Machine learning (ML) and data science (DS) are complex fields that can be difficult for people without a background in these areas to understand. Semantic interactions may offer a more accessible way to guide machine learning models without being forced to dive into technical details. However, there is a lack of research that examines whether the affordances offered by semantic interactions meet the expectations of domain experts who work with ML models. In this blog post, we will discuss our findings from an elicitation study we conducted using visual design probes to elicit how semantic interactions refine ML models.



In semi-structured interviews with 20 participants, we captured and summarized semantic interactions as a set of target-action pairs. For example, one participant stated that they would want to be able to "drag variables around on the graph so I can see how they interact" in order to better understand how the model works. This type of interaction allows users direct manipulations of data visualizations which can then be used feedback loops within machine learning algorithms for improved performance . Participants also expected a visual analytics system , such as IBM SPSS Modeler or KNIME Analytics Platform , to perform a speculative execution in response to actions; participants wanted to be able to review the effects of their interactions in realtime .



Overall, our findings suggest that semantic interactions offer domain experts another avenue through which they can refine ML models. These types of interactions provide users with more control over how data is displayed and allow them make immediate changes based on their observations . As such, semantically interactive systems may help reduce some cognitive load associated with working with ML models



==> tex/theory.tex <==
\section{A Theoretical Framework of Semantic Interactions}
This section reflects on our findings and the properties of semantic interactions that we elicited from our studies. From these findings, we motivate the need to develop more formal theories for semantic interactions. We propose a way to describe semantic interactions using a consistent notation, delineate their properties, and integrate them into ML model refinement. 

\subsection{Theoretical Motivations}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/processes_visual.pdf}
    \caption[]{Illustration of using user refinements ($\tau$) to refine a machine learning model. Here, we have an example of just two refinements: changing the label via the color encoding channel ($\tau_1$) and subsequently modifying the size encoding of the mark ($\tau_2$) to refine the predicted probability. These semantic interactions modify the visual representations ($\Delta R$) and can be passed as input to refine the ML model. This illustration of a model refinement is intentionally simplistic, but a user can take multiple actions (i.e., change color, size, and position of a mark).}
    \label{fig:process_summary}
\end{figure*}

We observed that prior research proposing frameworks for semantic interactions and interference tend to occupy two different levels of detail. At a high level, prior research presents frameworks that constitute a person interacting with a visualization and that this is change by humans and then captured by a machine learning model. In these high-level descriptors, there is not often a description of an intermediary mechanism for how this information is transmitted. Alternatively, other works propose low-level and specific mechanisms that are specific to the application context~\cite{SPERRLE:coadative:2021,sacha:2017:wywc} 

We strove to develop a framework for semantic interactions that can act as a middle layer between the high-level frameworks and application specific techniques for semantic interactions. Our framework comprises a notation for describing semantic interactions and also delineating their properties. Next, we describe the mechanisms for existing systems using this framework.  Kim~\cite{Kim2015InteractiveAI}  introduced the idea of `interacted latent variables' and defined them as a type of variable that is ``inferred from both human feedback and the data''. We leverage this idea to incorporate semantic interactions into ML model refinement.

\subsection{Describing Semantic Interactions}
Figure~\ref{fig:process_summary} presents our notations for semantic interactions via direct manipulations of visual encodings together with examples of interactions from our study (~\autoref{fig:results_main}).

Semantic interactions have four primary components: the dataset that is input to the model, the initial model specifications, the visualization of the model outputs, and finally, the interaction mechanisms by the end-user.

We denote the dataset provided to the model using the notation $D$. Applying a machine learning model to this data to generate an output, for example, predicting movie genres or a set of topics, augments the initial dataset, which we denote as $D'$.

The initial model specifications consist of those parameters provided by the end-user as input and are set (or learned) by the model training process. We denote the parameters of the machine learning model by the notation of $\theta$. We can further break these down according to whether the end-user provided them, $\theta_{U}$, or learned, $\theta_{M}$. For example, an end-user might specify the initial number of clusters in a topic model, which we consider to be $\theta_{U}$, while other parameters of the model are learned $\theta_{M}$. Another way to define these parameters is as observed ($\theta_{U}$) and latent ($\theta_{M}$) of the model. 

We use the $R$ notation to represent the visualization of the model outputs. We use $R$ because we consider this to be a visual representation of the model; we use this term precisely to align our terminology with the notions of embedded representations that are routinely visualized as part of the model inspection process~\cite{Demiralp:embeddings:2014}. We consider visual representations to have two states. The first state $R_{0}$ is the initial visual representation, which is either produced by the analyst or generated automatically by the system. For example, in a system like ForceSpire, the spatialized representation is automatically generated. The second state of the visualization has been modified by the end-user, $R_{1}$. The difference between these two states, $\Delta R$, can inform the updating of the model parameters.

Finally, we use the $\tau$ notation to denote the user interactions. Kindlmann et al.~\cite{Kindlman:2014} chose $\alpha$ and $\omega$ to represent changes to the data and visualization, respectively, because they bookend the start and the end of a visualization process. We choose $\tau$, the greek symbol associated with life, to denote user interactions in this same spirit. In semantic interactions, $\tau$ modifies the visual representation as follows : $R_0 \overset{\tau}{\rightarrow} R_1$. 

The intervention-action pairs in~\autoref{fig:results_main} show the relationships between different semantic interactions ($\tau$) and their modification of the visual representations ($\Delta R$). Moreover, we also show the intended target (intervention) of the semantic interaction, which can be within $D$ (initial labels) or $D'$ (probabilities, predicted labels, and clusters).


\subsection{Properties of Semantic Interactions}\label{subsec:ref_actions}
In addition to enumerating the intervention-action pairs, we also summarize a set of properties for semantic interactions. In our notation, these are properties of $\tau$.

\vspace{1mm}
\noindent\textbf{Semantic Interactions  are Targeted.} People do not apply model refinements to arbitrary examples from the data or result set. Instead, we saw evidence that people use an internal frame of reference when deciding upon what marks to target and, importantly, how they choose to make a refinement. In our study, participants articulated this frame of reference in what we called `degrees of wrongness' and familiarity with the data. While other studies have indicated that participants show data or feature prioritization when refining a model and actively use this information in model updates, we are the first to articulate a specific strategy for prioritization. 

We observed that both data familiarity and `wrongness' were important to prioritize semantic interactions. Even in our study, where participants had only a passing familiarity with the movie dataset, they exhibit a targeted search behavior. With completely unfamiliar datasets, where individuals with no contextual knowledge of its content would not prioritize the order and type of semantic interactions. An example of such a scenario could be providing a lay person with a dataset of measurements from a physics experiment without any data dictionaries or other forms of explanations. We do not know the frequency that people analyze datasets that are totally unfamiliar to them and while we suspect it is not common, we do believe this is an interesting observation to test in future work. This observation should also be carefully considered in future studies seek to use generic datasets such as mtcars or the iris data to evaluate their systems -- study participants level of familiarity with the data and this could effect their assessment of the systems.

\vspace{1mm}
\noindent\textbf{Semantic Interactions are Fuzzy.} Participants expressed that their feedback should not be interpreted precisely by an ML model but as suggestions with some degree of uncertainty. 
Through our visual probes, we found that different encoding choices naturally conveyed a sense of input uncertainty. Positional channels and text were perceived to have greater precision, whereas size and color refinements did not. These fuzzy inputs also let participants add their subjective ideas about what is important in the data. For example, in modifying a mark in a scatter plot, non-ML:06 stated ``\textit{I am not worried about giving too big numbers [via size encoding] to the model. Like if Wayne’s World [mark size] is too big, that is just me speaking my truth}.'' 
This finding also points to exciting opportunities to extend prior research on uncertainty visualization~\cite{padilla:2020:uncertainty}, which has primarily focused on communicating uncertainty \textit{to people} toward effectively transmitting uncertainty \textit{from people} to the model. 


\vspace{1mm}
\noindent\textbf{Semantic Interactions are Compounded.} Attributes in ML model results are correlated and should change together. For example, if an individual modifies the genre by changing the color, this action impacts the classification probability, and the size of the point should adjust.  Study participants were quick to make this observation. For example, participant non-ML:05 stated that when they ``move a point to a new genre, I expect the probability to be higher''. The converse is true when participants modified the probability; they wanted the label to update. Another example of a compounded action was in the scatter chart, where participants wanted to use distance from a cluster center to adjust the model's output probability and the movie genre.

\vspace{1mm}
\noindent\textbf{Semantic Interactions are Hierarchical.} Participants did not limit themselves to refining individual marks that encoded movie data. They also sought to refine movie genres themselves and have those actions pass down to individual movie marks. For example, if the participant expanded the boundaries of a mark representing a genre, then they would want all movie marks affected by this change to have their predicted labels and classification probabilities also adjust, but automatically. Participants also wanted to introduce data hierarchies that did not exist in the data. For example, three participants indicated that they wanted to indicate certain movie marks as more important than others to a genre and should act as an anchor for the genre. As participants moved points within a cluster, they wanted the classification probability to be adjusted relative to this anchor.




\subsection{Incorporating Semantic Interactions into Model Refinement}

We bring together our notation for semantic interactions and their properties to discuss prior approaches for semantic interactions and their gaps. We then propose a mechanism of using `interacted latent variables,' described previously by Kim~\cite{Kim2015InteractiveAI} to capture semantic interactions. 

\noindent\textbf{Describing Semantic Interactions of Prior Systems} 
A baseline reference is a system with input widgets, such as slides or input boxes, enabling an end-user to supply a parameter value directly. This parameter value can be, for example, the number of genres a model should predict or the minimal size of a cluster. These control widgets supply values for $\theta_{U}$ at model initialization. This approach is ubiquitous, but, as many prior works have already described (Section~\ref{sec:relatedwork}), they also limit how end-users can interact with a machine learning model. 

Semantic interactions that the ForceSpire~\cite{Endert:2012:SemanticOG} system supports would primarily modify the dataset $D$ and the feature space (the words). Modifications to $D$, for example, up-weighting a document, do not directly affect model parameters. However, changing the weights to the features does, since they are a direct part of the model parameters ($\theta_{M}$). Adjusting the feature weights directly through user interactions has been used by others. For example, an approach by Kumar et al.~\cite{kumar2019didn} directly updates priors on words through interactions with visualizations. More recent work by El-Assady et al.~\cite{el-assady_progressive_2018} can provide a more sophisticated way of learning feature weights using re-enforcement learning. Their approach involves the comparison of two models to fine-tune model $\theta_{M}$ progressively. 

This prior research demonstrates that semantic interactions can influence ML model refinement through either $D$ or $\theta_M$. Moreover, they emphasize how targeted interactions can steer model refinement while compensating for some overfitting. However, we argue that these prior works do not demonstrate a way to address other properties of semantic interactions that we surfaced in our study. For example, it is not clear how these systems would handle the end-user having different degrees of confidence in their interactions (i.e., whether a document belongs to one or more topics to varying degrees), compounded actions (i.e., proximity to a cluster centroid and the label of a point), or hierarchical actions (i.e., collapsing multiple clusters together, instead of making document level changes).

The semantic inference via probabilistic ML hooks proposed by Gehrmann et al.~\cite{Gehrmann:MLhooks:2020} are a more promising approach. However, this method too would primarily influence $\theta_M$ through modifications to $D$ by ``deciding what content is important'' through a hook network. %The specific example used by Gerhmann et al. consists of simulating all possible sequences of words given some input. 
Moreover, in Gerhmann et al.'s notion of collaborative semantic interactions, the end-user essentially provides more entities to update the model. However, the benefit of their probabilistic approach is that the model can is trained incrementally, as posteriors are used as input to the next refinement cycle. This incremental approach is similar to El-Assady's progressive updates, albeit with a different mechanism. However, we argue that there are some advantages to taking a more probabilistic approach over El-Assady's reinforcement learning strategy to incorporate semantic interactions' fuzzy and hierarchical properties. We see a possibility to extend ML-Hooks to incorporate hyperpriors, which are themselves probability distributions that act on the latent variables ($\theta_M$). This so-called multi-level modeling is a common bayesian approach~\cite{Allenby:hiearchal_bayes:2005} and could be leveraged for semantic interactions. Changes in visual representation ($\Delta_R$) could theoretically be used to fit those hyperpriors; that visual encodings can convey different degrees of confidence (Section~\ref{sec:full_study}) can enable this uncertainty to be directly modeled from $\Delta_R$ via hyper priors.

Overall, we find that prior methods are capable, in varying degrees, of handling the properties of semantic interactions that we observed in our study. However, there remains a conceptual leap between the existing capabilities of these systems and how they might be extended to better accommodate these properties, for example, using hyperpriors. As a final component of our framework for semantic interactions, we propose the use of `interacted latent variables'~\cite{Kim2015InteractiveAI} to augment existing techniques for semantic interactions. 


%\begin{figure}[h!]
%    \centering
%    \includegraphics[width=0.45\textwidth]{figures/framework_simple.pdf}
%    \caption{}
%    \label{fig:simple_framwork}
%\end{figure}


\vspace{1mm}
\noindent\textbf{Capturing Semantic Interactions as \textit{Interacted Latent Variables}.}
From the previous subsection, we can surmise that human feedback is incorporated in two ways. One way is by directly changing values of an observed variable ($\theta_U$) through control widgets or elements of the data, such as labeled genres. Another, is by augmenting the original dataset and influence the `latent' variables are learned entirely from the data and represent unmeasured constructs, for example, topics in a topic model. Kim~\cite{Kim2015InteractiveAI} introduced the notion of an `interacted latent variable' as a middle ground between latent and observed variables. Leveraging idea that human interactions with data are `fuzzy', this new variable type balances human input against what it learned from the data.
%Kim~\cite{Kim2015InteractiveAI}  introduced the idea of `interacted latent variables' and defined them as a type of variable that is ``inferred from both human feedback and the data''. By comparison, `latent' variables are learned entirely from the data and represent unmeasured constructs, for example, topics in a topic model. Observed variables are directly measured or o

In our experiment, the movie genre is an example of an `interacted latent variable.' Although labels were part of the original dataset, participants still wanted to modify them and convey a degree of uncertainty in their changes. We argue that the nature of the modifications was governed by the participants' mental models of movies. Although this mental model of the data is not observed, we believe it can be indirectly modeled through refinements introduced by semantic interactions.  

Another surprising `interacted latent label' was the predictive probability of the model. The participants want certain movies to be predicted with some specific probability. Again, \textit{Die Hard} is a good example of such a film, where participants wanted to convey that the movie should be split between `Action' and `Holiday' genres. While several factors are involved in computing this predictive probability, it may be possible to trace the effects of a semantic interaction on one or model latent variables.

Lastly, we argue that `interacted latent variables' can satisfy the properties of our observed semantic interactions. Like many of the previous systems, they can leverage prioritized actions of end-users to update the model incrementally. As we will describe in the next paragraph, they can also directly accept input from the end-user that has some degree of uncertainty. Finally, they can be leveraged as hyperpriors or even replace existing latent variables to address semantic interactions' hierarchical and compounded properties. 


\vspace{1mm}
\noindent\textbf{Refining an ML model through Interacted Latent Variables.} Kim outlines a three-step inference pipeline for incorporating human feedback that applies to semantic interactions. Roughly paraphrased, the first step is to ascertain how confident the person is in their feedback, the second is to propagate that feedback to the ML model based on that level of confidence, and the third step is to balance this feedback against what the model learns solely from the data. The idea is to let the high confidence human feedback override what is learned from the data and otherwise let the data drive. Kim's approach explicitly asks how confident they are in their feedback and uses a threshold that determines when human feedback supersedes the input data.%, but we think it is possible to instead (or even jointly) use $\Delta R$ to determine the trade-off between human feedback and the data. 

We propose using the magnitude of $\Delta R$ to manage this trade-off, either instead of or jointly with a person explicitly indicating the level of confidence of their feedback. For example, consider a scenario where a person wants to change the predicted genres of movies. If they change only a single data point than $\Delta R \approx 0$, this small change should indicate that the human feedback should be discounted relative to what is learned from the data. If the person feels that a movie must be predicted in some specific way, they could do so by modifying the mark's channel (perhaps changing its shape) or using other interface elements to communicate this. Alternatively, if a person makes many changes, resulting in a $\Delta R > 0$, then human feedback can take more precedence over what is learned from the data.  We could use a threshold for $\Delta R$, as Kim's method would, or could even be adaptively learned through successive rounds of feedback. Balancing this trade-off is a design decision that a visualization researcher or practitioner must make. Different strategies can exist for calculating $\Delta R$; we see this as a potent area of future research.  %Moreover, depending on the strategy chosen, it may be necessary to add additional random variables to the IGM to capture desired changes. By delineating the structure of IGMs, we intend to provide a scaffold for others to make those decisions, one that is both more concrete and generalizable relative to the frameworks and instances of specific systems in Section~\ref{sec:relatedwork}. 

%To refine the ML model, we would take the difference between these two data representations, $R_1 - R_0$, propagate this information through the model in the manner that Kim proposes~\cite{Kim2015InteractiveAI}. Again, we emphasize the visualization and ML designers still need to fine-tune how this data is incorporated for specific models and types of data, but this notation for an interactive graphical model serves as a scaffold for this process.

